S stars and s-process in the Gaia era II. Constraining the luminosity of the third dredge-up with Tc-rich S stars

S stars are late-type giants that are transition objects between M-type stars and carbon stars on the asymptotic giant branch (AGB). They are classified into two types: intrinsic or extrinsic, based on the presence or absence of technetium (Tc). The Tc-rich or intrinsic S stars are thermally-pulsing (TP-)AGB stars internally producing s-process elements (including Tc) which are brought to their surface via the third dredge-up (TDU). Tc-poor or extrinsic S stars gained their s-process overabundances via accretion of s-process-rich material from an AGB companion which has since turned into a dim white dwarf. Our goal is to investigate the evolutionary status of Tc-rich S stars by locating them in a Hertzsprung-Russell (HR) diagram using the results of Gaia early Data Release 3 (EDR3). We combine the current sample of 13 Tc-rich stars with our previous studies of 10 Tc-rich stars to determine the observational onset of the TDU in the metallicity range [-0.7; 0]. We also compare our abundance determinations with dedicated AGB nucleosynthesis predictions. The stellar parameters are derived using an iterative tool which combines HERMES high-resolution spectra, accurate Gaia EDR3 parallaxes, stellar evolution models and tailored MARCS model atmospheres for S-type stars. Using these stellar parameters we determine the heavy-element abundances by line synthesis. In the HR diagram, the intrinsic S stars are located at higher luminosities than the predicted onset of the TDU. These findings are consistent with Tc-rich S stars being genuinely TP-AGB stars. The comparison of the derived s-process abundance profiles of our intrinsic S stars with the nucleosynthesis predictions provide an overall good agreement. Stars with highest [s/Fe] tend to have the highest C/O ratios.

==> Li.tex <==
\section{Derivation of the Li abundance}

%\LS{IS THIS SECTION REFERENCED SOMEWHERE ?}

%\LSrm{I WOULD REMOVE THESE PARAGRAPHS}{ The main production mechanism for $^7$Li is believed to be the Cameron-Fowler (CF) mechanism, in which an enrichment of $^3$He follows the first dredge-up episode. The excess $^3$He may reach the inner stellar layers, where it is burned to form $^7$Be, which leads to the production of $^7$Li. When a low-mass star evolves to become a cool giant, the standard evolution model predicts that Li will be significantly diluted by a factor of about 60 after the first dredge-up \citep{Iben1967}. Li decreases further because of mixing after the RGB bump \citep{sweigart1979}. Though evolved stars in general are considered as Li sinks, AGB stars are known to produce fresh Li \citep{smithandlambert1989} via the CF mechanism. It is understood that Li production in AGB stars happens only in relatively massive stars of M $\ge$ 3 \msun~through hot bottom burning (HBB, \cite{mowlavi1995}).}

%\LSrm{}{The discovery of high Li abundance in relatively less evolved low-mass RGB stars was unexpected \citep{wallerstein1982}. \cite{kovari2013} and \cite{lyubimkov2012} found Li-rich F, G, K type giants from their Li abundance analysis. The super Li-rich carbon stars from \cite{abia1991} show Li abundances 10 to 100 times higher than the present cosmic values. The excess of Li found in some stars is really puzzling. There have been several theories to explain the Li enrichment like non-standard mixing, accretion of nova ejecta or engulfment of a planet. Despite of the efforts, the disagreement between the predicted and observed Li abundances in AGB/RGB stars still remains a question \citep{casey2019}.}

%\LSrm{}{In an attempt to bridge the gap in our understanding of Li abundances in AGB stars} 
We 
%derived Li abundances 
used the Li~I line at 6707.8 \AA. 
%From their study of oxygen-rich AGB variables, \cite{uttenthaler2010} found that this Li line is usually blended with the neighbouring contributions from Ce \SVE{**Which Ce line? which ionization stage? Can you specify? **}. --> Have removed this because in UTH they find that the contribution cant be from Ce line.
In Fig.~\ref{fig:Liexample} we present examples for stars with a good (bottom panel) as well as bad (top panel) 
spectral synthesis fitting the  considered Li line.
We could derive the Li abundance for only three stars from our sample, namely HR~Peg, V679~Oph and Vy~12. For these stars, the absorption features at the Li doublet located at 6707.8~\AA~are very clear, for the rest of the sample there were severe blends in the Li line (top panel of Fig.~\ref{fig:Liexample}) so only upper limits on the Li abundances could be derived. The data are listed in Table ~\ref{tab:Liabund}. 
%It is a bit strange that in fig A.1 you illustrated a good fit and a bad fit, but none is used to derive a Li abundance, both are used to derive limits. I would have expected a good fit, leading to an abundance (HR~Peg, V679~Oph and Vy~12) and a bad fit, leading to an upper limit.

The Li abundances of all the intrinsic S stars of our sample are generally low except for HR~Peg. HR~Peg was found to be a Li-rich star also by \cite{vanture2007} who classified the star as a high-mass star (M > 3\msun) with HBB as an explanation to the Li abundance. However, from our derivations of masses, HR~Peg has $M_\mathrm{curr}$ = 2.1~\msun{} which is in agreement with the mass estimates by other authors in literature \citep[2.0~\msun{} from][]{pieter2015}. So HR~Peg is not sufficiently massive to be producing Li though HBB. The other plausible explanations %discussed in several works are
invoke some extra mixing in low-mass AGB stars \citep[e.g.][]{charbonnel2000, uttenthaler2007,uttenthaler2010} or the engulfment of planets/brown dwarfs \citep{Siess99}.


%\subsubsection{Infrared colours and Tc}\label{InfraVSTc}
%\begin{figure}
%    \centering
%   \includegraphics[scale=0.35]{InfraredexcessVslogTc_fullsample_3.png}
%    \caption{Infrared excess as a function of Tc abundance. The ratio R was calculated using the color-corrected IRAS flux at 12 and 2.2 $\mu$m listed in Table~\ref{table:infraredexcess}. The circles represent the photometric variability retrieved from ASAS and AAVSO whenever available.}
%    \label{fig:InfraVsTc}
%\end{figure}
%As a star evolves on the TP-AGB its mass loss and infrared excess increase \citep{guandalini2010}. Even if S stars are not among the most evolved TP-AGB objects, a correlation might already be present. In  Fig.~\ref{fig:InfraVsTc}, we compare the infrared excess, 
%\SVE{computed as in \shreeya{\cite{pieter2015}}, } with the Tc abundances. 
% in Fig.~\ref{fig:InfraVsTc}. 
%We find a strong 
%\textbf{We did not find any trend of increasing Tc abundances with increasing infrared excess.
%for the majority of objects.
%In fact in Fig.~\ref{fig:InfraVsTc}, there are four stars with very high infrared excess but relatively low Tc abundance compared to the rest of our sample. These stars are located in the upper left corner of Fig.~\ref{fig:InfraVsTc} (at R $> 0.075$)  
%except for 4 outliers in the left corner of
%are 
%namely 
%HR~Peg, V915~Aql, CSS~154 and CD~-29~5912. As can be seen from Table~\ref{table:infraredexcess} and Fig.~\ref{fig:InfraVsTc}, these stars also have high photometric variability, which can lead to an increase in the infrared excess \citep{guandalini2010} while the Tc abundance is still low as they are not much evolved on the TP-AGB (Fig.~\ref{HRD})}. %\SG{I thought we excluded those stars with $\Delta V >1$ from the sample !? cf Sect. 2}
%\textbf{possible explanations for this?? high temperatures in the interiors destroying the Tc? high dilution in the convective envelope?}


%\begin{table*}[]
%\caption{Column 2 presents the Tc abundance for all the sample stars and for the Tc-rich stars from S18, S19 and S20a. Column 3  gives the flux at f(12~$\mu$m) from the IRAS Point source catalog v2.1 calibrated using the correction factor at 3000~K (Correction factor = 1.41). The f(2.2~$\mu$m) in column 4 was calculated using K$_{2MASS}$ magnitude. Infrared excess ratio R is f(12~$\mu$m)/f(2.2~$\mu$m). In column 6 we list the photometric variability ($\Delta V$) collected from AAVSO and the All Sky Automated Survey (ASAS). Column 7 lists the mass loss rates retrieved from literature whenever available. }
%    \centering
%    \begin{tabular}{l|c c c c c c}
%    \hline
%         Star & $\log \epsilon_\mathrm{Tc}$ & f(12) & f(2.2) & R = f(12)/f(2.2) & $\Delta V$ & $\dot{M}$ (Reference)   \\
%         & & Jy & Jy & & mag & \msun/yr \\
%         \hline
%         HR Peg & -1.3 & 19.57 & 255.58 & 0.076 & 0.9 & < $6.3 \times 10^{-8}$ \citep{jorissen1998}\\
%         HD 288833 & -1.2 & 0.65 & 13.14 & 0.049 & 0.2 & - \\
%         V812 Oph & 1.0 & 1.169 & 16.63 & 0.070 & 1.4 & - \\
%         AA Cam & -0.4 & 10.31 & 185.32 & 0.055 & - & $3.83 \times 10^{-8}$ \citep{ramstedt2009} \\
%         V1139 Tau & -0.6 & 17.32 & 270.85 & 0.063 & 0.6 & - \\
%         KR CMa & & 5.74 & 109.42 & 0.052 & 0.7 &  - \\
%         CSS~151 & -0.1 &  0.56 & 9.219 & 0.060 & 0.5 & - \\
%         CD -27 5131 & & 4.98 & 54.091 & 0.092 & 1.0 & $4.7 \times 10^{-8}$ \citep{jura1988} \\
%         BD -18 2608 &  -0.1 & 0.938 & 16.456 & 0.057 & - \\
%         V679 Oph & 0.5 & 3.144 & 55.760 & 0.056 & 0.8 & $3.3 \times 10^{-8}$ \citep{jura1988} \\
%         CSS 454 & 0.5 & 0.420 & 7.078 & 0.059 & 0.5 & - \\
%         CSS~1152 & 0.5 & 1.529 & 20.85 & 0.073 & - & - \\
%         HD 64147 & -0.1 & 1.351 & 23.962 & 0.056 & 0.5 & - \\
%         \hline
%         Omi Ori & -0.4 & 60.53 & 1226.67 & 0.049 & 0.2 & < $2.0 \times 10^{-7}$ \citep{jorissen1998} \\
%         BD +79 156 & -0.7 & 0.525 & 10.128 & 0.051 & - & - \\
%         V915 Aql & -0.2 & 7.76 & 97.25 & 0.079 & 1.0 & $4.6 \times 10^{-8}$ \citep{jura1988} \\
%         UY Cen & & & & & 2.6 & $2.1 \times 10^{-7}$ \citep{jorissen1998} \\
%         NQ Pup & -0.3 & 4.97 & 79.71 & 0.062 &1.0 & $6.3 \times 10^{-7}$ \citep{jorissen1998}\\
%         HD 357941 & -0.2 & 2.72 & 51.80 & 0.052 & 0.6 & - \\
%         CSS 154 & -0.6 & 1.56 & 20.26 & 0.077 & 0.6 & - \\
%         CSS 182 & 0.0 & 0.856 & 13.168 & 0.065 & 0.5 & -  \\
%         CD -29 5912 & -0.6 & 0.495 & 6.431 & 0.076 & 1.3 & -  \\
%         BD +34 1698 & -0.6 & 1.328 & 21.975 & 0.060 & - & -  \\
%         \hline
%    \end{tabular}
%    \label{table:infraredexcess}
%\end{table*}


1315 	& HR Peg &S4+/1+&	 6.36 &	 0.94 &	 2.15 &	 2.35 $\pm$	 0.16 & 0.11 & 2.93 & 17 July 2009 &   60      \\
233          & HD 288833 &S3/2  & 9.40  & 4.26  & 5.51  & 0.84 $\pm$ 0.05 & 0.19 & 2.84  &20 August 2012 &      100   \\
%114          & omi Ori &M3SIII    & 4.72 & -0.66 & 0.48  & 6.16 $\pm$ 0.41 & 0.07 & 2.91   & 29 January 2010 &      200   \\
997          & V812 Oph&S5+/2.5  & 10.58 & 4.00  & 5.22  & 0.78 $\pm$ 0.07 & 0.18 & 2.93  & 22 April 2016 & 40         \\
%CSS 1219 & V* V441 Cyg &S4,6  & 9.80         & 1.772 & 3.367  & 1.3688 $\pm$ 0.0809 & 0.09    & &      \\
%CSS 1254 & V* V2141 Cyg &MS & 7.48         & 1.333 & 2.587  & 1.9287 $\pm$ 0.0983 &  0.085   & &    \\
%CSS 347          & V* Y Lyn &M6S    & 6.98  & -0.44  & 0.88   & 2.9657 $\pm$ 0.2841 &  0.252  & &         \\
312          & AA Cam & M5S    & 7.79  & 1.39  & 2.59  & 1.84 $\pm$ 0.06 & 0.07 & 2.84   & 9 April 2011 & 90        \\
89           & V1139 Tau&S & 7.90  & 0.97  & 2.27  & 1.81 $\pm$ 0.13 &  0.16 & 3.00   & 23 November 2012 & 150       \\
265          & KR CMa&M4S    & 8.50  & 1.96  & 3.30  & 1.42 $\pm$ 0.06 & 0.18 & 3.01    &10 April 2011 & 70        \\
%CSS 856          & V* R Cam &S2    & 9.74  & 2.455  & 3.822  & 0.7897 $\pm$ 0.0536 &  0.084   & &       \\
151          & CSS 151    &S  & 10.99 & 4.64  & 5.97  & 0.48 $\pm$ 0.07 &  0.10 & 2.91   &31 July 2017 &    40   \\
474          & CD -27 5131 &S4,2 & 9.62  & 2.72  & 4.35  & 0.56 $\pm$ 0.05 & 0.13 & 3.01 & 2 April 2010 & 70    \\
%CSS 471          & CSS 471  &S & 10.48  & 4.174  & 5.445  & 0.6569 $\pm$ 0.0822 & 0.142 & &  \\
597          & BD -18 2608 &S & 9.58   & 4.01  & 5.27  & 0.77 $\pm$ 0.05 &0.10 & 2.91 & 24 March 2018 & 70   \\
%CSS 932          & BD+07 3210 &S & 9.55   & 4.377  & 5.498  & 0.5023 $\pm$ 0.0470  & 0.084 & &  \\
1070 &  V679 Oph & S5/5+ & 8.92         & 2.69 & 4.16  & 1.16 $\pm$ 0.06 & 0.08 & 2.83 & 16 March 2018 & 80        \\
%106          & BD +79 156 &S4/2  & 9.55   & 4.54  & 5.67  & 0.57 $\pm$ 0.03  & 0.26 & 2.85 & 1 December 2009 & 60  \\
454          & CSS 454 &S  & 10.39  & 4.93  & 6.13  & 0.63 $\pm$ 0.07 & 0.12 & 2.91 & 2 February 2017 & 50 \\
1152 & CSS 1152 & S5-/6        & 10.13        & 3.76 & 5.06  & 0.62 $\pm$ 0.04  & 0.07 & 2.99 &  18 March 2018 & 80   \\
416          & HD 64147&S5/2.5 & 9.20   & 3.61  & 5.00  & 0.58 $\pm$ 0.07 & 0.06 & 2.93 & 27 November 2016 &40\\
%CSS 511         & CD -29 6206 & S4*1 & 10.66   & 6.753  & 5.554  & 0.4574 $\pm$ 0.0333 & 0.208 & 21 February 2018 & 50\\



\begin{table}[]
    \centering
    \begin{tabular}{c c c c}
CSS &          Star        & DR2 parallax $\pm$ error   & eDR3 parallax $\pm$ error \\
89           & V1139 Tau   & 1.81 $\pm$ 0.13            & 1.79 $\pm$ 0.04  \\
151          & CSS 151     & 0.48 $\pm$ 0.07            & 0.36 $\pm$ 0.02 \\
233          & HD 288833   & 0.84 $\pm$ 0.05            & 0.83 $\pm$ 0.02\\
265          & KR CMa      & 1.42 $\pm$ 0.06            & 1.29 $\pm$ 0.02 \\
312          & AA Cam      & 1.84 $\pm$ 0.06            & 2.08 $\pm$ 0.05\\
416          & HD 64147    & 0.58 $\pm$ 0.07            & 0.56 $\pm$ 0.02\\
454          & CSS 454     & 0.63 $\pm$ 0.07            & 0.40 $\pm$ 0.03  \\
474          & CD -27 5131 & 0.56 $\pm$ 0.05            & 0.64 $\pm$ 0.03\\
597          & BD -18 2608 & 0.77 $\pm$ 0.05            & 0.71 $\pm$ 0.02 \\
997          & V812 Oph    & 0.78 $\pm$ 0.07            & 0.64 $\pm$ 0.03 \\
1070         &  V679 Oph   & 1.16 $\pm$ 0.06            & 1.04 $\pm$ 0.03 \\
1152         & CSS 1152    & 0.62 $\pm$ 0.04            & 0.58 $\pm$ 0.02\\
1315 	     & HR Peg      & 2.35 $\pm$	 0.16           & 2.14 $\pm$ 0.08  \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

%New Tables with EDR3
\begin{table*}
\caption{\label{finalparams} Atmospheric parameters for S stars. %after performing iterations on \logg. 
%The metallicities [Fe/H] have been obtained from the  Fe abundance analyses. 
%\SVE{(Explain what is L, Lupp and Llow)} 
%\shreeya{I removed the columns for  $L_{\rm upp}$ and $L_{\rm low}$, I didn't like it alot. So I entered those values like we did for other paper and modified this caption to explain the values in brackets.} 
In the \teff\ and $\log g$ and [s/Fe] columns, the numbers between brackets denote the values spanned during the $\log g$ iterations, while in the C/O column they indicate the error on C/O from the CH regions and in the $L$ column, they indicate the luminosity error due to the Gaia DR2 error on the parallax.
The numbers in  brackets in the [Fe/H] column indicate the number of Fe lines used to derive [Fe/H] and the next column indicates the standard deviation (derived from the line-to-line scatter) on [Fe/H]. The current (M$_{\rm curr}$) and initial (M$_\mathrm{ini}$) masses have been derived from the locations of the stars in the HR diagram compared to STAREVOL tracks \shreeya{(Sect.~\ref{sectHRD})}.} %\SVE{3 decimals should be mentioned in this table for C/O! the third decimal IS relevant for S star spectra!}}
\centering %
\setlength\tabcolsep{4pt}
\begin{tabular}{l c c  c l l c c c c}
%\setlength\extrarowheight{4pt}
\hline 
 Name & $T_{\rm eff}$ & $L$ &  $\log g$ & [Fe/H] &$\sigma_{\rm [Fe/H]}$& C/O & [s/Fe] & M$_{\rm curr}$ & M$_{\rm ini}$\\
  & (K) & ($L_{\odot}$) & (dex) & & & &(dex) &($M_{\odot}$)&($M_{\odot}$) \\
\hline \\
V1139 Tau & 3400 & 6600 & 1 & -0.06 (13) & 0.13 & 0.752 & 1 &  2.9 & 3.2\\
 & (3400 - 3500)  & (6300 - 6900) & (1 - 3)  & & & (0.500 - 0.752)  &(1 - 1))  & &  \\
CSS 151  & 3500 & 5900 & 1 & -0.25 (14) & 0.14 & 0.500  & 1  &  & \\
 & (3500 - 3600)  & (5300 - 6600) & (1 - 3)  & & & (0.500 - 0.899) &(1 - 1)  & &  \\
HD 288833 & 3600  & 1700 & 1 & -0.30 (13) & 0.14 & 0.500 & 0  &  1.2 & 1.4\\
 & (3600 - 3600)  & (1600 - 1800) & (1 - 2) & & & (0.500 - 0.752)  & (0 - 1) & &  \\
 KR CMa & 3400 & \textbf{5100} & \textbf{0}  & -0.01 (13) & 0.22 & 0.500 & 1  & 2.7 & 2.9 \\
 & (3400 - 3500)  & (4900 - 5400) & (1 - 3)  & & & (0.500 - 0.752) &(1 - 1)  & &  \\
AA Cam   & 3600 & 4800  & 1 & -0.32 (15) & 0.13 & 0.500  & 0  & 2.5 & 2.7 \\
 & (3600 - 3600) & (4500 - 5200) & (1 - 2)  & & & (0.500 - 0.899)  &(0 - 1)  & &  \\
HD 64147 & 3500  & 5600  & 0 & -0.67 (11) & 0.10 & 0.500  & 0 & 2.7 & 2.9\\
 &(3500 - 3600)  & (4400 - 7300) &(0 - 1)  & & & (0.500 - 0.752) &(0 - 1)  & &  \\
CSS 454 & 3500   & 1500 & 1 & -0.38 (12) & 0.14 & 0.500  & 1 & 0.7 & 1.0 \\
 & (3500 - 3600) & (1200 - 1900) & (1 - 3)  & & & (0.500 - 0.899) & (1 - 1)  & &  \\
CD -27\deg5131 & 3400 & 12900 & 0 & -0.30 (9) & 0.12 & 0.500 & 1 & 3.6 & 4.0\\
  &(3400 - 3600))  & (10600 - 16100) & (0 - 3) & & & (0.500 - 0.899)  &(1 - 1)  & &  \\
BD -18\deg2608 & 3500 & 2300 & 1 & -0.31 (13) & 0.16 & 0.752  & 1 & 1.3 & 1.5\\
 &(3500 - 3600)  & (2000 - 2600) & (1 - 3)  & & & (0.500 - 0.899)  &(1 - 1)  & &  \\
V812 Oph & 3500 & 2300 & 1  & -0.37 (13) & 0.13 & 0.500 & 1 & 1.2 & 1.4\\
  & (3500 - 3500)  & (1900 - 2800) & (1 - 2)  & & & (0.500 - 0.899) &(1 - 1)  & &  \\
V679 Oph   & 3600  & 3600 & 1 & -0.52 (9)  & 0.14 &  0.899 & 1 & 1.6 & 1.8\\
 &(3600 - 3600)  & (3300 - 4100) & (1 - 1) & & & (0.752 - 0.899)  &(1 - 2)  & &  \\ 
CSS 1152 & 3400  & 4100 & 1 & -0.14 (6) &0.13 &0.971  & 1 & 2.5 & 2.6 \\
 &(3400 - 3600) & (3600 - 4700) & (1 - 2)  & & & (0.899 - 0.971) &(1 - 2)  & &   \\
HR Peg     & 3500  & 4100  & 0  & -0.34 (13)  & 0.17 & 0.500 & 0  & 2.1 & 2.2 \\
 & (3500 - 3600) & (3600 - 4800) & (0 - 4)  & & & (0.500 - 0.752)  & (0 - 1)  & & \\
\hline
\end{tabular}
%\captionsetup{justification=centering}
\end{table*}


%Copy of the table with eDR3 relative difference
\begin{table*}
\caption{\label{basic data} Basic data for our S star sample. Columns 1 and 2 list different identifiers: CGSS \citep[]{cgss}   entry number and HD, BD or other names. Columns 3, 4, 5, and 6 indicate spectral type, $V$, $J$ and $K$ magnitudes, respectively, extracted from the SIMBAD Astronomical Database \citep{simbad}. Column 7 lists the Gaia DR2 parallax and its error. Column 8 lists the relative difference, which is $(|\varpi_{\rm DR2} - \varpi_{\rm eDR3}|)/ \varpi_{\rm eDR3}$. The reddenning $E_{B-V}$ has been obtained from the \cite{gontcharov} extinction maps. $BC_K$ is the bolometric correction in the $K$ band as computed from the MARCS model atmospheres. Columns 10 and 11 document the HERMES spectra observation dates 
%of the HERMES spectra 
and their signal-to-noise (S/N) ratio estimated around 500 nm.}
\centering
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{r l l c c c c c c c c c}
\hline
%\rule{0pt}{20pt}
 CSS & Name & Sp. type & $V$ & $J$ & $K$ & \multicolumn{1}{c}{$\varpi_{\rm DR2}\pm\sigma_{\varpi}$} & $\myfrac{|\varpi_{\rm DR2} - \varpi_{\rm eDR3}|}{\varpi_{\rm eDR3}}$ & $E_{(B-V)}$ & $BC_{K}$ & Observation date & S/N \\
  & & & & & & (mas) & & & & & \\
\hline
89           & V1139 Tau&S & 7.90  & 0.97  & 2.27  & 1.81 $\pm$ 0.13 & 0.01  &0.16 & 3.00   & 23 November 2012 & 150       \\
151          & CSS 151    &S  & 10.99 & 4.64  & 5.97  & 0.48 $\pm$ 0.07 & 0.33 & 0.10 & 2.91   &31 July 2017 &    40   \\
233          & HD 288833 &S3/2  & 9.40  & 4.26  & 5.51  & 0.84 $\pm$ 0.05 & 0.01 & 0.19 & 2.84  &20 August 2012 &      100   \\
265          & KR CMa & M4S    & 8.50  & 1.96  & 3.30  & 1.42 $\pm$ 0.06 & 0.10 & 0.18 & 3.01    &10 April 2011 & 70        \\
312          & AA Cam & M5S    & 7.79  & 1.39  & 2.59  & 1.84 $\pm$ 0.06 & 0.11  & 0.07 & 2.84   & 9 April 2011 & 90        \\
416          & HD 64147&S5/2.5 & 9.20   & 3.61  & 5.00  & 0.58 $\pm$ 0.07 & 0.03 & 0.06 & 2.93 & 27 November 2016 &40\\
454          & CSS 454 &S  & 10.39  & 4.93  & 6.13  & 0.63 $\pm$ 0.07 & 0.57 & 0.12 & 2.91 & 2 February 2017 & 50 \\
474          & CD -27\deg5131 &S4,2 & 9.62  & 2.72  & 4.35  & 0.56 $\pm$ 0.05 & 0.12 & 0.13 & 3.01 & 2 April 2010 & 70    \\
597          & BD -18\deg2608 &S & 9.58   & 4.01  & 5.27  & 0.77 $\pm$ 0.05 & 0.08 & 0.10 & 2.91 & 24 March 2018 & 70   \\
997          & V812 Oph&S5+/2.5  & 10.58 & 4.00  & 5.22  & 0.78 $\pm$ 0.07 & 0.22  & 0.18 & 2.93  & 22 April 2016 & 40         \\
1070 &  V679 Oph & S5/5+ & 8.92         & 2.69 & 4.16  & 1.16 $\pm$ 0.06 & 0.10  & 0.08 & 2.83 & 16 March 2018 & 80        \\
1152 & CSS 1152 & S5-/6        & 10.13        & 3.76 & 5.06  & 0.62 $\pm$ 0.04  & 0.06 & 0.07 & 2.99 &  18 March 2018 & 80   \\
1315 	& HR Peg &S4+/1+&	 6.36 &	 0.94 &	 2.15 &	 2.35 $\pm$	 0.16 & 0.09  & 0.11 & 2.93 & 17 July 2009 &   60      \\
\hline
\end{tabular}
\end{table*}
\renewcommand{\arraystretch}{1}
